Interpretability in Parameter Space: Minimizing Mechanistic Description Length with Attribution-based Parameter Decomposition

Mechanistic interpretability aims to understand the internal mechanisms learned by neural networks. Despite recent progress toward this goal, it remains unclear how best to decompose neural network parameters into mechanistic components. We introduce Attribution-based Parameter Decomposition (APD), a method that directly decomposes a neural network's parameters into components that (i) are faithful to the parameters of the original network, (ii) require a minimal number of components to process any input, and (iii) are maximally simple. Our approach thus optimizes for a minimal length description of the network's mechanisms. We demonstrate APD's effectiveness by successfully identifying ground truth mechanisms in multiple toy experimental settings: Recovering features from superposition; separating compressed computations; and identifying cross-layer distributed representations. While challenges remain to scaling APD to non-toy models, our results suggest solutions to several open problems in mechanistic interpretability, including identifying minimal circuits in superposition, offering a conceptual foundation for 'features', and providing an architecture-agnostic framework for neural network decomposition.

==> _Background.tex <==





==> deprecated_discussion.tex <==
\section{Discussion}%


We propose APD, a method for decomposing networks into mechanistic components directly in parameter space. Our implementation works on a range of toy models and has a range of potential advantages over existing techniques. Nevertheless, certain challenges, such as sensitivity to hyperparameters, will need to be overcome before the method can be used reliably. We identify a number of future research directions that may address current issues.  


\subsection{Advantages of our approach}
\paragraph{Parameter space interpretability engages more directly with what we care about} Our approach attempts to decompose the network into components directly in parameter-space. This is quite different from the Sparse Dictionary learning-based approach of decomposing neural activations and then linking them up into circuits (TODO cite, maybe Sam Marks?). We think parameter space interpretability might be preferable and could potentially solve a lot of the problems with the SDL paradigm. Decomposing the model itself instead of its activation spaces gives us access to a lot more relevant information: With activation-space interpretability, we do not necessarily know which directions in an activation space the model itself treats as significant at the time we choose them (TODO Lee, cite might be good.). We only know what directions look sparse or special in the data itself. This makes it difficult to choose directions that will yield simple model components we can more easily reverse-engineer, since we cannot directly optimise the directions to have simple interactions. Decomposing the model into components allows us to directly optimise for obtaining simple model components.
\paragraph{Representations can be higher dimensional and span multiple layers}SDL methods currently in use assume that features are always one-dimensional (TODO cite), but evidence suggests representations in language models are at least sometimes better described as multi-dimensional \cite{engels2024languagemodelfeatureslinear}. Likewise, there has been concern about how to deal with cross-layer representations and cross-layer superposition (Lee help, cite Anthropic update?). Our method is natively capable of dealing with both of these problems, since parameter components can be multidimensional and span many layers.
\paragraph{Decomposing parameters directly may bypass the issue of feature geometry}Since our method does not involve a prerequisite step of decomposing the model’s activations, it might allow us to decompose models accurately without needing to understand their feature geometry first. This seems like a potential big advantage. Feature geometry appears to be rich and complex. (TODO Lee cite) 
It might be hard to unravel the geometry if we don't know yet what computations the geometry is trying to enable. After all, it's hard to define what a `feature' of the activations even is if we don't know yet what the model does with the activations (TODO Cite would be great here if available). 
But if we already have an accurate decomposition, we could then try to understand the feature geometry by reasoning about the ways different circuits interact, using the residual stream activations to exchange information. 
\paragraph{Connections to the nascent science of deep learning} Since mechanisms are defined directly in parameter space, it might be easier to relate them to theories of neural network training that analyze the structure of the loss landscape, such as those based on Singular Learning Theory \citep{watanabe2009algebraic, Hoogland_Murfet_Oldenziel_Wingerden_2023}.




\subsection{Current limitations}
\paragraph{Hyperparameter sensitivity} The largest issue at the moment is that the optimization appears to be quite sensitive to hyperparameters. Extensive fine-tuning was often required to get a decomposition working, and some imperfections in the resulting components tended to persist even then. Our aim with this work was to develop a theoretically well grounded mechanistic decomposition method rather than a method that is immediately practical for real-world models. Making the method more robust is one of our highest priorities for future work.
\paragraph{APD is not indifferent to layer structure}
We want to find components in the structure of the learned network algorithm, rather than the network architecture. 
Thus, we would prefer our formalism to be entirely indifferent to changes of network parameterization that do not affect the underlying algorithm. 
However, APD is currently not indifferent to changes of network parameterization that mix network layers. 
This is because we optimize parameter components to be simple by penalizing them for being high rank, and the rank of weight matrices cannot be defined without reference to the network layers. 
Thus, if two components in different neural networks implement essentially the same computation, one in a single layer, the other in cross-layer superposition, the latter component may be assigned a higher rank. Thus, while we think that APD can still find components that stretch over many layers, it may struggle to do so more than for components that stretch over fewer layers. 
To solve this problem, we are thinking about replacing the rank of APD components with other layer-invariant quantities that more accurately track the simplicity of components independent of their parametrization. Speculatively, some variation of the weight-refined local learning coefficient \cite{wang2024differentiationspecializationattentionheads} might fulfill this requirement. 


\paragraph{Decomposition is based solely on coactivation} The APD criterion for decomposing networks into components is based solely on component coactivation, not component connectivity (TODO maybe cite something on the latter notion of module/component). If two parts of a model are always used for the same input, APD would not separate them into two components even if they are disconnected from each other and do not interact at all. To further decompose such parts into even smaller components, post-processing with different decomposition methods might be needed. However, how necessary this is in practice remains unclear at the moment. (TODO maybe elaborate why?)
\paragraph{Computational costs at scale may be high} A potential problem for our method is its computational cost. For frontier models, the cost scaling might be comparable to or even higher than the cost of Sparse Dictionary methods such as Sparse Autoencoders. In the worst case, assuming networks made of a vast ensemble of very very small parameter components, perfect recovery might cost around $\mathcal{O}(L^2 d^3)$ operations per forward pass, where $L$ is the number of weight matrices and $d$ is their dimensionality. This is worse than the worst-case assumption for end-to-end SAEs \cite{braun2024identifying} in a similar scenario, which would be ca. $\mathcal{O}(L d^3)$\footnote{This estimate is based on information theory constraints on the maximal number of distinct operations that can be specified in a neural networks' parameters \cite{adler2024complexityneuralcomputationsuperposition}, \cite{Bushnaq_Mendel_2024}.} There may be techniques to reduce the cost of the method, but these make additional assumptions about the structure of models that would need to be validated first. See Appendix \ref{appendix:eff_meth} for details.






\subsection{Future work}
\paragraph{Improving attributions} We currently use attribution patching to estimate the importance of parameter components for computing the network's output. There might be better attribution methods available. For example, gradient-attribution becomes inaccurate when weight gradients become small due to a saturated softmax, or other functions implemented by the network that have small derivative. This problem could be alleviated by using integrated gradients instead \cite{sundararajan2017axiomatic}.
\paragraph{More toy models (TODO)} Additional experiments we plan to carry out include making the toy model of polysemantic computation multi-layer, decomposing a network with components that differ a lot in rank to test that APD is robust to this, decomposing a toy model that makes use of attention and decomposing a single MLP layer of a small language model. %
\paragraph{Using APD results to motivate better intrinsic interpretability architectures}: If APD proves to be too expensive to use for decomposing increasingly larger frontier models, using it on smaller models might still yield insights into how high-performing models are structured internally. This might help develop more performant, intrinsically interpretable architectures like improved Mixture of Experts (TODO cite) setups. This would lower the alignment tax for using interpretable architectures, potentially making them a more feasible choice for frontier models.



\section{appendix comp efficiency discussion}
\section{More efficient implementations of APD} 
\label{appendix:eff_meth}
The APD method involves training $C$ parameter vectors of the same size as the original network $\theta\in \mathbb{R}^N$. How large $C$ will need to be in real models is unclear at this stage. In the worst case, it could be information-theoretically possible for a network to consist of an extremely large ensemble of small components, such that $C$ is of the same order as the number of parameters in the original model $C=\mathcal{O}(N)$ \citep{adler2024complexityneuralcomputationsuperposition}. 

However, there are some alleviating factors that we think might reduce the computational cost significantly, depending on how the mechanistic internals of frontier models turn out to be structured. It is thus somewhat unclear to us at the moment whether running APD on frontier models will turn out to be more expensive, comparable, or less expensive than training a set of Sparse Autoencoders for every layer of the model. 

\paragraph{Low-rank components}(Already implemented and working)
We would often expect the components $P_c$, to correspond to low-rank matrices, particularly when the total number of components $C$ is large low-rank structures correspond to simpler components that are easier to fit into the original model. At the extreme, if $C=\mathcal{O}(N)$, we would expect most components to be rank-$1$ matrices. On the other hand, if many components are high rank, then we expect there to be fewer components in total because there is no room to fit them into the model parameters otherwise \citep{Bushnaq_Mendel_2024}. For example, if a component has the same rank as the original model in every layer, we would expect that this is the only model component, and the network cannot be broken up further. This is useful because it might often allow us to parametrize most components as low-rank matrices from the start, greatly reducing computational costs. 

If real models proved to mostly consist of many very simple components, one might even attempt to constrain all $P_c$ to be rank-$1$ matrices, to begin with, then cluster coactivating sets of components together into higher rank components afterward where appropriate. 

We have already used low-rank parameterizations to reduce the computational costs for running APD on several of the toy models presented in this paper.








\paragraph{Component hierachies} 
Some components may themselves be composed of other components, forming a hierarchy. In this case, we can save on computing by performing the APD decomposition hierarchically as well. For example, imagine a network that is composed of $100$ large components, each of which are themselves composed of $100$ smaller components, each which is in turn composed of $100$ very small elementary components. Then, instead of calculating attributions for $10^6$ elementary components and selecting the active ones, we could calculate attributions for $100$ macro-components, select the $k_1<<100$ largest ones, perform a second attribution calculation on their set of $100k_1$ sub-components, select the $k_2<<100k_1$ largest ones, then finally calculate attributions for $100k_2$ elementary components and select the $k_3<<100k_2$ largest ones to perform the sparse forward pass and update their parameters based on the result. In this way, we can greatly reduce the cost of the attribution calculation and gradient update, which are the most expensive operations in APD. How large the cost reduction is would depend on how hierarchical the structure of the network's components is.



==> multilayer_linear.tex <==

\subsection{Sanity check of APD on cross-layer distributed representations: Multilayer Linear model}\label{app:deep-linear}
\todo{(Dan) Either remove or fix with rank-penalty and standard sparse dataset}Given an input vector $x \in R^d$ of $d$ sparsely activating data features, we train a multi-layer linear network (i.e. without any non-linearities, residual stream, or embedding matrices) to implement an identity mapping, outputting $y^L=x$ at the last layer. The network consists of $L$ layers of matrices $W^l \in \mathbb{R}^{d\times d}$. While $W^L \dots W^2 W^1=1$ has to multiply out to an identity, intermediary hidden activations can be rotated and distorted relative to the input, e.g. $W^2 W^1 x \neq x$, in general. 

We would expect this network to be separable into $d$ sparsely activating components, with each component encompassing the weights that connect a particular input feature to the directions it is represented in throughout the network layers. This should mean that each parameter component traces out a single `path' through the model, mapping a particular feature from one layer to the next. So we should find that each component corresponds to a rank one matrix at every layer, with the rank one matrix in the very first layer being a single row connecting to a single input feature, and the rank one matrix in the last layer being a single column connecting to a single output feature. As shown in Figure \ref{fig:deep-linear-params}, APD indeed finds the desired solution.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{deep_linear_params.png}
    \caption{Learned parameter components of a 3-layer linear network (no non-linearities) with $W^l\in\mathbb{R}^{5\times 5}$, after training APD with $5$ parameter components. The components become approximately rank one matrices, following a single feature from the network input to the output.}
    \label{fig:deep-linear-params}
\end{figure}

